Algorithm for Invalidation of Cached Results of Queries to a Single Table

One of the most popular setups for a back-end of a high performance website consists of a relational database and a cache which stores results of performed queries. Several application frameworks support caching of queries made to the database, but few of them handle cache invalidation correctly, resorting to simpler solutions such as short TTL values, or flushing the whole cache after any write to the database. In this paper a simple, correct, efficient and tested in real world application solution is presented, which allows for infinite TTL, and very fine grained cache invalidation. Algorithm is proven to be correct in a concurrent environment, both theoretically and in practice.

==> conclusion.tex <==
%auto-ignore



==> tmp <==
\title{Algorithm for Invalidation of Cached Results of Queries to a Single Table}
\author{
  Jakub Łopuszański \footnote{
    Department of Computer Science and Mathematics, University of Wrocław
  }
}
\date{}
\maketitle

